Port-Hamiltonian multibody dynamics: Lagrangian formulation, consistent interconnection, structure-preserving simulation and index-reduction

This work introduces a port-Hamiltonian (PH) model for constrained mechanical systems, which is directly derived from the Lagrangian equations of motion. The present PH framework incorporates a singularity-free director representation of rigid body rotations, resulting in constant mass matrices. It is shown that the power-preserving interconnection of PH rigid-body subsystems is mathematically equivalent to the classical description of ideal joints using kinematic pairs. This establishes a PH multibody dynamics framework that is consistent with traditional modeling paradigms. Notably, the PH structure of the governing index-2 differential-algebraic equations enables the application of an implicit, structure preserving midpoint time integration. The proposed scheme is able to satisfy both the balance laws for total energy and angular momentum as well as the position-level constraints. These properties make the proposed method remarkably robust and enable stable long-term simulations. Furthermore, a variationally derived index-reduction strategy is incorporated that enforces velocity-level constraints in addition to position-level constraints while preserving the port-Hamiltonian structure. Numerical examples illustrate the favorable properties of the proposed formulation, which is well-suited for energy-based control design.

==> drawings/interconnection.tex <==
%% Creator: Inkscape 1.4.2 (f4327f4, 2025-05-13), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'interconnection.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{507.93895331bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.20276353)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{drawings/interconnection.pdf}}%
    \put(0.06121159,0.16474159){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}2 continuous PHS \eqref{eq:joint-interconnection-separate-bodies}\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{drawings/interconnection.pdf}}%
    \put(0.66450319,0.16469401){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}1 continuous PHS \eqref{eq:interconnected-system}\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{drawings/interconnection.pdf}}%
    \put(0.7055673,0.01969717){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}1 discrete PHS \eqref{eq:discretized_eqs_full}\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{drawings/interconnection.pdf}}%
    \put(0.12495118,0.01969717){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}2 discrete PHS\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{drawings/interconnection.pdf}}%
    \put(0.0,0.09175665){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\footnotesize Discretization \eqref{eq:port_hamiltonian_form_discrete} \end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=6]{drawings/interconnection.pdf}}%
    \put(0.39331197,0.18921498){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\footnotesize  Interconnection \eqref{eq:PH-interconnection-port-matrices-2} \end{tabular}}}}%
    \put(0.80623767,0.09175665){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\footnotesize  Discretization \eqref{eq:port_hamiltonian_form_discrete} \end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=7]{drawings/interconnection.pdf}}%
    \put(0.39331197,0.04521613){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\footnotesize Interconnection \eqref{eq:discrete-transformer-interconnection} \end{tabular}}}}%
  \end{picture}%
\endgroup%


==> includes/annex_old.tex <==
%########################################################################
\section*{Appendix}\label{annexsec:annex}
%########################################################################

\section{Balance of angular momentum for the director rigid body} \label{app_ang_mom}

For ease of analysis, we consider an individual rigid body as described in \eqref{eq:ph_constraint_compact_simple} with total angular momentum \eqref{eq:angular_momentum_rigid_body}. Its time derivative reads
\begin{equation}
    \dot{\vec{L}} = \boldsymbol{\varphi} \times  m \ddot{\vec{\varphi}}  + \sum_{i=1}^{3} \vec{d}_i \times  E_i \ddot{\vec{d}}_i,
    \label{eq:balance_angular_momentum}
\end{equation}
due to the vanishing cross-product of a vector with itself. Considering the rigid body's equations of motion
\begin{subequations} \label{eq:multibody_system_equations_of_motion}
\begin{align}
        \dot{\boldsymbol{\varphi}}&= \bm{v}_{\boldsymbol{\varphi}}, \label{eq:evolution_position_trans_mbs}\\
        \dot{\bm{d}}_i  &= \bm{v}_{\bm{d}_i}, \label{eq:evolution_position_rot_mbs}\\
        m \dot{\bm{v}}_{\boldsymbol{\varphi}} &= -\nabla V(\boldsymbol{\varphi}) + \bm{f}_{\boldsymbol{\varphi}}, \label{eq:evolution_velocity_trans_mbs}\\
        E_i \dot{\bm{v}}_{\bm{d}_i} &= -\nabla\, \bm{g}_\text{d}(\bm{d}_i)^\top\,\bm{\lambda} \bm{f}_i, \label{eq:evolution_velocity_rot_mbs}\\
    \nabla \bm{g}(\bm{d}_i)\: \bm{v}_{\bm{d}_i} & = \bm{0}, \label{eq:director_constraints_mbs}
\end{align}
\end{subequations}
we insert \eqref{eq:evolution_velocity_trans_mbs} and \eqref{eq:evolution_velocity_rot_mbs} into \eqref{eq:balance_angular_momentum}. We further consider co-linearity of constraint forces and directors such that $\vec{f}^\mathrm{d}_i \times \vec{d}_i = \vec{0} $ and obtain
\begin{align}
    \dot{\vec{L}} =-\boldsymbol{\varphi} \times \nabla V(\boldsymbol{\varphi})+ \boldsymbol{\varphi}\times \vec{f}_{\boldsymbol{\varphi}}+ \vec{d}_i \times \vec{f}_i,
    \label{eq:balance_angular_momentum2}
\end{align}
showing that in the absence of external and potential forces, angular momentum is conserved. In the case of active gravitational forces, e.g. $\nabla V (\boldsymbol{\varphi})=- m g\, \vec{e}_3$, the component of the angular
momentum in the $\vec{e}_3$-direction remains constant, i.e. $\frac{\text{d}}{\text{d}t}(\vec{L}\transp \vec{e}_3)=0$.

In discrete time, the angular momentum balance can be shown to hold true for the discrete evolution equations \eqref{eq:port_hamiltonian_form_discrete} as well.
If applied to the rigid body formulation
the scheme is given by
\begin{subequations} \label{eq:discretized_eqs_full}
    \begin{align}
        \boldsymbol{\varphi}^{n+1} - \boldsymbol{\varphi}^n                                    & = h\, \vec{v}_{\boldsymbol{\varphi}}^{n+\frac{1}{2}}, \label{eq:discretized_eq_translational_com}                                                                                                             \\
        \vec{d}_i^{n+1} - \vec{d}_i^n                                                          & = h\, \vec{v}_{\vec{d}_i}^{n+\frac{1}{2}} \quad \text{for} \ i=1, 2, 3 , \label{eq:discretized_eq_rotational_com}                                                                                             \\
        m \left(\vec{v}_{\boldsymbol{\varphi}}^{n+1} - \vec{v}_{\boldsymbol{\varphi}}^n\right) & = -h\, \nabla V(\boldsymbol{\varphi}^{n+\frac{1}{2}})  +h\,\vec{f}_{\boldsymbol{\varphi}}^{n+\frac{1}{2}}, \label{eq:discretized_eq_translational_d}                                                          \\
        E_i \left(\vec{v}_{\vec{d}_i}^{n+1} - \vec{v}_{\vec{d}_i}^n\right)                     & = -h\, \nabla \vec{g}(\vec{d}_i^{n+\frac{1}{2}})\transp \vec{\lambda}_\text{d}^{n+\frac{1}{2}} + h\,\vec{f}_{\vec{d}_i}^{n+\frac{1}{2}} \quad \text{for} \ i=1, 2, 3 , \label{eq:discretized_eq_rotational_d} \\
        \nabla \vec{g} (\vec{d}_i^{n+\frac{1}{2}})\, \vec{v}_{\vec{d}_i}^{n+\frac{1}{2}}       & = \vec{0} .  \label{eq:discretized_eq_constraint}
    \end{align}
\end{subequations}

We now show that the discrete-time formulation under the midpoint rule also yields an angular momentum balance.
Evaluating the continuous angular momentum balance \eqref{eq:balance_angular_momentum}
at $t^n$ and $t^{n+1}$ yields
\begin{equation}
    \begin{aligned}
        \vec{L}(\vec{x}^{n+1})  - \vec{L}(\vec{x}^n) =  \vec{\varphi}^{n+1} \times m \vec{v}_{\boldsymbol{\varphi}}^{n+1} - \vec{\varphi}^{n} \times m\vec{v}_{\boldsymbol{\varphi}}^{n}  +  \vec{d}_i^{n+1} \times E_i \vec{v}_{\vec{d}_i}^{n+1} - \vec{d}_i^{n} \times E_i \vec{v}_{\vec{d}_i}^{n} .
    \end{aligned}
    \label{eq:change_angular_momentum}
\end{equation}
To evaluate each term, we use the standard identity
\begin{equation}
    \begin{aligned}
        \scriptscriptstyle \mathbf{a}^{n+1} \times \mathbf{b}^{n+1} - \mathbf{a}^n \times \mathbf{b}^n = \frac{1}{2}  \left[\left( \mathbf{a}^{n+1} - \mathbf{a}^n \right) \times  \left( \mathbf{b}^{n+1} + \mathbf{b}^n \right) +  \left( \mathbf{a}^{n+1} + \mathbf{a}^n \right) \times \left( \mathbf{b}^{n+1} - \mathbf{b}^n \right)\right] .
    \end{aligned}
    \label{eq:cross_product_difference}
\end{equation}
Applying \eqref{eq:cross_product_difference} to the translational term in \eqref{eq:change_angular_momentum} and substituting the discrete evolution laws \eqref{eq:discretized_eq_translational_com} and \eqref{eq:discretized_eq_translational_d} yields
\begin{equation}
    {\scriptscriptstyle
        \vec{\varphi}^{n+1} \times m\vec{v}_{\boldsymbol{\varphi}}^{n+1} - \vec{\varphi}^{n} \times m\vec{v}_{\boldsymbol{\varphi}}^{n}=
        \frac{h}{2} \left[ \left( \vec{v}_{\boldsymbol{\varphi}}^{n+1} + \vec{v}_{\boldsymbol{\varphi}}^{n} \right) \times \left( m \vec{v}_{\boldsymbol{\varphi}}^{n+1} + m \vec{v}_{\boldsymbol{\varphi}}^{n} \right)
            - \left( \vec{\varphi}^{n+1} + \vec{\varphi}^{n} \right) \times \nabla V\left( \vec{\varphi}^{n+\frac{1}{2}} \right) + \left( \vec{\varphi}^{n+1} + \vec{\varphi}^{n} \right) \times \vec{f}_{\boldsymbol{\varphi}}^{n+\frac{1}{2}}\right] .}
    \label{eq:change_translational_momentum_2}
\end{equation}
The first term vanishes due to the collinearity of the velocity vector with itself. A similar expansion for the director term results in
\begin{equation}
    {\scriptscriptstyle
        \vec{d}_i^{n+1} \times E_i\, \vec{v}_{\vec{d}_i}^{n+1} - \vec{d}_i^{n} \times E_i \,\vec{v}_{\vec{d}_i}^{n}=
        h\left[\frac{1}{2} \left( \vec{v}_{\vec{d}_i}^{n+1} + \vec{v}_{\vec{d}_i}^{n} \right) \times  \left(  E_i \vec{v}_{\vec{d}_i}^{n+1} +  E_i \vec{v}_{\vec{d}_i}^{n} \right)
            -  \vec{d}_i^{n+\frac{1}{2}}  \times \nabla \vec{g}( \vec{d}_i^{n+\frac{1}{2}})\transp\vec{\lambda}^{n+\frac{1}{2}} + \vec{d}_i^{n+\frac{1}{2}}  \times \vec{f}_{\vec{d}_i}^{n+\frac{1}{2}}\right].}
    \label{eq:change_rotational_momentum_2}
\end{equation}
Again, the first term vanishes due to collinearity, and the second vanishes due to collinearity of constraint forces and directors.
Combining both contributions yields
\begin{equation}
    \vec{L}(\vec{x}^{n+1})  - \vec{L}(\vec{x}^n) = - h \left[ \vec{\varphi}^{n+\frac{1}{2}}  \times \nabla V\left( \vec{\varphi}^{n+\frac{1}{2}} \right)- \vec{\varphi}^{n+\frac{1}{2}} \times \vec{f}_{\boldsymbol{\varphi}}^{n+\frac{1}{2}}-\,\vec{d}_i^{n+\frac{1}{2}}  \times \vec{f}_{\vec{d}_i}^{n+\frac{1}{2}}\right].
    \label{discrete_angmom_balance}
\end{equation}
Thus, if no external potential or external loads act on the system, the right-hand side vanishes, and angular momentum is exactly conserved under the midpoint rule.

%########################################################################
\section{Derivation of constraint gradient from a PH port matrix}\label{annexsec:technical-details-PH-interconnection}
%########################################################################

An interconnected multibody system can also be formulated directly as a single PH-DAE system according to \eqref{eq:ph_constraint_compact_simple}. By comparing both formulations, one can identify the equivalence of the two approaches.
Equating \eqref{eq:relation-port-matrix-constraint-gradient} with the last row of the PH-DAE formulation \eqref{eq:ph_constraint_compact_simple}, one gets the equivalence \eqref{eq:joint_cons_vel_bulk}, which is given here again for convenience as
\begin{align}
\begin{bmatrix}
        -\tilde{\vec{B}}_\text{int}^{A\transp} & \tilde{\vec{B}}_\text{int}^{B\transp}
    \end{bmatrix}
    \begin{bmatrix}
        \vec{v}^A \\
        \vec{v}^B
    \end{bmatrix}
    = \nabla \vec{g}_{\text{J}}(\vec{q}) \vec{v}. 
    \label{eq:constraint-gradient-from-port-matrix}
\end{align}
Specifically, it can be deduced that the velocity-related part of the internal port matrices $\tilde{\vec{B}}_\text{int}^{\alpha}$
acts on the velocities in the same way as the gradient of \eqref{eq:cylindrical-pair-constraints}, which is given by the $4 \times 24$ matrix
\begin{align}
    \nabla \vec{g}_{\text{J}}^C(\vec{q}) =
    \begin{bmatrix}
        -\vec{m}_1^{A\transp} & \nabla \vec{g}_{11}\transp     & \nabla \vec{g}_{12}\transp     & \nabla \vec{g}_{13}\transp     & \vec{m}_1^{A\transp} & X_1^B \vec{m}_1^{A\transp} & X_2^B \vec{m}_1^{A\transp} & X_3^B \vec{m}_1^{A\transp} \\
        -\vec{m}_2^{A\transp} & \nabla \vec{g}_{21}\transp     & \nabla \vec{g}_{22}\transp     & \nabla \vec{g}_{23}\transp     & \vec{m}_2^{A\transp} & X_1^B \vec{m}_2^{A\transp} & X_2^B \vec{m}_2^{A\transp} & X_3^B \vec{m}_2^{A\transp} \\
        \vec{0}\transp        & n_1^{A} {\vec{d}_1^{B}}\transp & n_2^{A} {\vec{d}_1^{B}}\transp & n_3^{A} {\vec{d}_1^{B}}\transp & \vec{0}\transp       & {\vec{n}^{A}}\transp       & \vec{0}\transp             & \vec{0}\transp             \\
        \vec{0}\transp        & n_1^{A} {\vec{d}_2^{B}}\transp & n_2^{A} {\vec{d}_2^{B}}\transp & n_3^{A} {\vec{d}_2^{B}}\transp & \vec{0}\transp       & \vec{0}\transp             & {\vec{n}^{A}}\transp       & \vec{0}\transp
    \end{bmatrix},
    \label{eq:cylindrical-pair-constraint-jacobian}
\end{align}
where $ \nabla \vec{g}_{\alpha i} = (m_\alpha^A)_i \Delta \vec{p} - X_i^A \vec{m}_\alpha^A$,
for $\alpha = 1,2$ and $i = 1,2,3$.

%########################################################################
\subsection{Velocity-related port matrices cylindrical pair} \label{annexsubsec:port-matrices-cylindrical-pair}
%########################################################################
Let us first focus on the left-hand side of \eqref{eq:relation-port-matrix-constraint-gradient}.
We summarize here the velocity-related parts of the port matrices for bodies $A$ and $B$ such that from the general form \eqref{eq:external_force_input_generalized_force} we have
\begin{align}
    \tilde{\vec{B}}^A \vec{u}= \begin{bmatrix}
                                   \vec{I}                                             & \vec{0}                           \\
                                   -\frac{1}{2}\widehat{\vec{d}}^A_1 \widehat{\vec{r}}_1\ladd{^A} & -\frac{1}{2}\widehat{\vec{d}}^A_1 \\
                                  -\frac{1}{2}\widehat{\vec{d}}^A_2 \widehat{\vec{r}}_2\ladd{^A} & -\frac{1}{2}\widehat{\vec{d}}^A_2 \\
                                 -\frac{1}{2}\widehat{\vec{d}}^A_3 \widehat{\vec{r}}_3\ladd{^A} & -\frac{1}{2}\widehat{\vec{d}}^A_3 
                               \end{bmatrix} \begin{bmatrix}
                                                 \vec{F} \\
                                                 \vec{\tau}
                                             \end{bmatrix}, \qquad
    \tilde{\vec{B}}^B \vec{u}= \begin{bmatrix}
                                   \vec{I}                                             & \vec{0}                           \\
                                   -\frac{1}{2}\widehat{\vec{d}}^B_1 \widehat{\vec{r}}_1\ladd{^B} & -\frac{1}{2}\widehat{\vec{d}}^B_1 \\
                                  -\frac{1}{2}\widehat{\vec{d}}^B_2 \widehat{\vec{r}}_2\ladd{^B} & -\frac{1}{2}\widehat{\vec{d}}^B_2 \\
                                 -\frac{1}{2}\widehat{\vec{d}}^B_3 \widehat{\vec{r}}_3\ladd{^B} & -\frac{1}{2}\widehat{\vec{d}}^B_3 
                               \end{bmatrix} \begin{bmatrix}
                                                 \vec{F} \\
                                                 \vec{\tau}
                                             \end{bmatrix}. 
    \label{eq:PH-interconnection-port-matrices}
\end{align}
Following our cylindrical joint convention (joint frame defined with respect to $A$), the additional lever $\Delta \vec{p}$ (see \eqref{eq:cylindrical-pair-constraints}) from relative motion in the unconstrained direction contributes fully to the torque on $A$. \ladd{This results in the following lever vectors between the external force application point and the respective body's center of mass}
\begin{align}
    \vec{r}_i^A  = X_i^A \vec{d}_i^A + \Delta \vec{p} \qquad \qquad \vec{r}_i^B = X_i^B \vec{d}_i^B .
    \label{eq:lever-arm-annex_A_B}
\end{align}
\dadd{Moreover, it can be shown by means of the principle of virtual work that the external forces $\vec{f}_i =  -\frac{1}{2}X_j \widehat{\vec{d}}_i \widehat{\vec{d}}_j \vec{F} $ admit the equivalent representation} \cite{betsch2013}
\begin{align}
    \vec{f}_i = X_i \vec{F} . \label{tmp_equiv}
\end{align}
\ladd{Inserting \eqref{eq:lever-arm-annex_A_B} into \eqref{eq:PH-interconnection-port-matrices} and using \eqref{tmp_equiv},}
we obtain
\begin{equation}
    \begin{aligned}
        \tilde{\vec{B}}^A \vec{u} & =
        \begin{bmatrix}
            \vec{I}                                                        & \vec{0}                           \\
            X_1^A \vec{I} - \widehat{\vec{d}}^A_1 \widehat{\Delta \vec{p}} & -\frac{1}{2}\widehat{\vec{d}}^A_1\\
            X_2^A \vec{I} - \widehat{\vec{d}}^A_2 \widehat{\Delta \vec{p}} & -\frac{1}{2}\widehat{\vec{d}}^A_2\\
            X_3^A \vec{I} - \widehat{\vec{d}}^A_3 \widehat{\Delta \vec{p}} & -\frac{1}{2}\widehat{\vec{d}}^A_3
        \end{bmatrix}
        \begin{bmatrix}
            \vec{F} \\  \vec{\tau}
        \end{bmatrix},     \qquad
        \tilde{\vec{B}}^B \vec{u} & =
        \begin{bmatrix}
            \vec{I}       & \vec{0}                           \\
            X_1^B \vec{I} & -\frac{1}{2}\widehat{\vec{d}}_1^B\\
            X_2^B \vec{I} & -\frac{1}{2}\widehat{\vec{d}}_2^B\\
            X_3^B \vec{I} & -\frac{1}{2}\widehat{\vec{d}}_3^B\\
        \end{bmatrix}
        \begin{bmatrix}
            \vec{F} \\ \vec{\tau}
        \end{bmatrix}.
    \end{aligned}
    \label{eq:PH-interconnection-port-matrices-2-annex}
\end{equation}

%\pcomment{Wie kommt man auf \eqref{eq:PH-interconnection-port-matrices-2-annex}?}

The input quantities $(\vec{F}, \vec{\tau})$ are so far expressed with respect to the inertial frame. Let us now transform them into the joint frame $C$ with the related rotation matrix
$\vec{R}^C = \begin{bmatrix} \vec{n}^A & \vec{m}_1^A & \vec{m}_2^A \end{bmatrix}$. Find the definitions of these vectors in Section~\ref{sec:interconnection}.

Moreover, consider the identity
\begin{equation}
    \begin{aligned}
        -\frac{1}{2}\widehat{\vec{d}}_i^A \vec{R}^C
        %& = -\frac{1}{2}\widehat{\vec{d}}_i^A \left(\vec{d}_j^C \otimes \vec{e}_j\right)                                                                                                                                                \\
         & = -\frac{1}{2} \widehat{\vec{d}}_i^A \left(\vec{n}^A \otimes \vec{e}_1 + \vec{m}_1^A \otimes \vec{e}_2 + \vec{m}_2^A \otimes \vec{e}_3\right)                           \\
        %  & = -\frac{1}{2}\left[\left(\widehat{\vec{d}}_i^A \vec{n}^A\right)\otimes \vec{e}_1 + \left(\widehat{\vec{d}}_i^A \vec{m}_1^A\right)\otimes \vec{e}_2 + \left(\widehat{\vec{d}}_i^A \vec{m}_2^A\right)\otimes \vec{e}_3 \right] \\
         & = - \frac{1}{2} \begin{bmatrix}
                               \widehat{\vec{d}}_i^A \vec{n}^A & \widehat{\vec{d}}_i^A \vec{m}_1^A & \widehat{\vec{d}}_i^A \vec{m}_2^A
                           \end{bmatrix},
    \end{aligned}
    \label{eq:refactor-skew-symmetric-vector}
\end{equation}

For notational convenience, we define
%\plk{This does not make sense (scalars vs matrices.)}
\[
    \tilde{\bm{X}}_i^A = X_i^A\vec{I} - \widehat{\vec{d}}_i^A \Delta \widehat{\vec{p}}.
\]
such that we eventually obtain the port matrices
\begin{equation}
    \begin{aligned}
        \tilde{\vec{B}}^A & =
        \begin{bmatrix}
            \vec{n}^A               & \vec{m}_1^A                                   & \vec{m}_2^A               & \vec{0} & \vec{0} & \vec{0} \\
            \tilde{\bm{X}}_1^A \vec{n}^A & \tilde{\bm{X}}_1^A \vec{m}_1^A                     & \tilde{\bm{X}}_1^A \vec{m}_2^A
                                    & -\frac{1}{2}\widehat{\vec{d}}_1^A \vec{n}^A
                                    & -\frac{1}{2}\widehat{\vec{d}}_1^A \vec{m}_1^A
                                    & -\frac{1}{2}\widehat{\vec{d}}_1^A \vec{m}_2^A \\
            \tilde{\bm{X}}_2^A \vec{n}^A & \tilde{\bm{X}}_2^A \vec{m}_1^A                     & \tilde{\bm{X}}_2^A \vec{m}_2^A
                                    & -\frac{1}{2}\widehat{\vec{d}}_2^A \vec{n}^A
                                    & -\frac{1}{2}\widehat{\vec{d}}_2^A \vec{m}_1^A
                                    & -\frac{1}{2}\widehat{\vec{d}}_2^A \vec{m}_2^A\\
            \tilde{\bm{X}}_3^A \vec{n}^A & \tilde{\bm{X}}_3^A \vec{m}_1^A                     & \tilde{\bm{X}}_3^A \vec{m}_2^A
                                    & -\frac{1}{2}\widehat{\vec{d}}_3^A \vec{n}^A
                                    & -\frac{1}{2}\widehat{\vec{d}}_3^A \vec{m}_1^A
                                    & -\frac{1}{2}\widehat{\vec{d}}_3^A \vec{m}_2^A
        \end{bmatrix}, \\
        \tilde{\vec{B}}^B & =
        \begin{bmatrix}
            \vec{n}^A       & \vec{m}_1^A                                   & \vec{m}_2^A       & \vec{0} & \vec{0} & \vec{0} \\
            X_1^B \vec{n}^A & X_1^B \vec{m}_1^A                             & X_1^B \vec{m}_2^A
                            & -\frac{1}{2}\widehat{\vec{d}}_1^B \vec{n}^A
                            & -\frac{1}{2}\widehat{\vec{d}}_1^B \vec{m}_1^A
                            & -\frac{1}{2}\widehat{\vec{d}}_1^B \vec{m}_2^A \\
            X_2^B \vec{n}^A & X_2^B \vec{m}_1^A                             & X_i^B \vec{m}_2^A
                            & -\frac{1}{2}\widehat{\vec{d}}_2^B \vec{n}^A
                            & -\frac{1}{2}\widehat{\vec{d}}_2^B \vec{m}_1^A
                            & -\frac{1}{2}\widehat{\vec{d}}_2^B \vec{m}_2^A \\
            X_3^B \vec{n}^A & X_3^B \vec{m}_1^A                             & X_i^B \vec{m}_2^A
                            & -\frac{1}{2}\widehat{\vec{d}}_3^B \vec{n}^A
                            & -\frac{1}{2}\widehat{\vec{d}}_3^B \vec{m}_1^A
                            & -\frac{1}{2}\widehat{\vec{d}}_3^B \vec{m}_2^A
        \end{bmatrix}.
    \end{aligned}
    \label{eq:PH-interconnection-port-matrices-joint-frame-2-annex}
\end{equation}

As relative motion along and rotation about the $\vec{n}^A$ direction are unconstrained for the cylindrical pair, we consider partition \eqref{eq:ph_link_internal_external_ports}
and focus on the internal components of~\eqref{eq:PH-interconnection-port-matrices-joint-frame-2-annex}
given by
\begin{equation}
    \begin{aligned}
        \tilde{\vec{B}}_\text{int}^{A} & =
        \begin{bmatrix}
            \vec{m}_1^A               & \vec{m}_2^A                                   & \vec{0} & \vec{0} \\
            \tilde{\vec{X}}_1^A \vec{m}_1^A & \tilde{\vec{X}}_1^A \vec{m}_2^A
                                      & -\frac{1}{2}\widehat{\vec{d}}_1^A \vec{m}_1^A
                                      & -\frac{1}{2}\widehat{\vec{d}}_1^A \vec{m}_2^A \\
            \tilde{\vec{X}}_2^A \vec{m}_1^A & \tilde{\vec{X}}_2^A \vec{m}_2^A
                                      & -\frac{1}{2}\widehat{\vec{d}}_2^A \vec{m}_1^A
                                      & -\frac{1}{2}\widehat{\vec{d}}_2^A \vec{m}_2^A \\
            \tilde{\vec{X}}_3^A \vec{m}_1^A & \tilde{\vec{X}}_3^A \vec{m}_2^A
                                      & -\frac{1}{2}\widehat{\vec{d}}_3^A \vec{m}_1^A
                                      & -\frac{1}{2}\widehat{\vec{d}}_3^A \vec{m}_2^A 
        \end{bmatrix}, \\
        \tilde{\vec{B}}_\text{int}^{B} & =
        \begin{bmatrix}
            \vec{m}_1^A       & \vec{m}_2^A                                   & \vec{0} & \vec{0} \\
            X_1^B \vec{m}_1^A & X_1^B \vec{m}_2^A
                              & -\frac{1}{2}\widehat{\vec{d}}_1^B \vec{m}_1^A
                              & -\frac{1}{2}\widehat{\vec{d}}_1^B \vec{m}_2^A \\
            X_2^B \vec{m}_1^A & X_2^B \vec{m}_2^A
                              & -\frac{1}{2}\widehat{\vec{d}}_2^B \vec{m}_1^A
                              & -\frac{1}{2}\widehat{\vec{d}}_2^B \vec{m}_2^A \\
            X_3^B \vec{m}_1^A & X_3^B \vec{m}_2^A
                              & -\frac{1}{2}\widehat{\vec{d}}_3^B \vec{m}_1^A
                              & -\frac{1}{2}\widehat{\vec{d}}_3^B \vec{m}_2^A
        \end{bmatrix}.
    \end{aligned}
    \label{eq:PH-interconnection-internal-port-matrices-joint-frame-annex}
\end{equation}
We then combine the transpose of these matrices to obtain the velocity-related part of the internal port matrix
for a cylindrical pair as the right-hand side of \eqref{eq:relation-port-matrix-constraint-gradient}. More explicitly, this yields
\begin{align}
    \left[\begin{smallmatrix}
                  -\vec{m}_1^{A\transp} & -\left(\tilde{\vec{X}}_1^A \vec{m}_1^A\right)\transp & -\left(\tilde{\vec{X}}_2^A \vec{m}_1^A\right)\transp & -\left(\tilde{\vec{X}}_3^A \vec{m}_1^A\right)\transp &\vec{m}_1^{A\transp} & \left(X_1^B \vec{m}_1^A\right)\transp & \left(X_2^B \vec{m}_1^A\right)\transp & \left(X_3^B \vec{m}_1^A\right)\transp \\
                  -\vec{m}_2^{A\transp} & -\left(\tilde{\vec{X}}_1^A \vec{m}_2^A\right)\transp & -\left(\tilde{\vec{X}}_2^A \vec{m}_2^A\right)\transp & -\left(\tilde{\vec{X}}_3^A \vec{m}_2^A\right)\transp& \vec{m}_2^{A\transp} & \left(X_1^B \vec{m}_2^A\right)\transp & \left(X_2^B \vec{m}_2^A\right)\transp & \left(X_3^B \vec{m}_2^A\right)\transp \\
                  \vec{0}\transp & \left(\tfrac{1}{2} \widehat{\vec{d}}_1^A \vec{m}_1^A\right)\transp & \left(\tfrac{1}{2} \widehat{\vec{d}}_2^A \vec{m}_1^A\right)\transp & \left(\tfrac{1}{2} \widehat{\vec{d}}_3^A \vec{m}_1^A\right)\transp & \vec{0}\transp & \left(-\tfrac{1}{2} \widehat{\vec{d}}_1^B \vec{m}_1^A\right)\transp & \left(-\tfrac{1}{2} \widehat{\vec{d}}_2^B \vec{m}_1^A\right)\transp & \left(-\tfrac{1}{2} \widehat{\vec{d}}_3^B \vec{m}_1^A\right)\transp \\
                  \vec{0}\transp & \left(\tfrac{1}{2} \widehat{\vec{d}}_1^A \vec{m}_2^A\right)\transp & \left(\tfrac{1}{2} \widehat{\vec{d}}_2^A \vec{m}_2^A\right)\transp & \left(\tfrac{1}{2} \widehat{\vec{d}}_3^A \vec{m}_2^A\right)\transp & \vec{0}\transp & \left(-\tfrac{1}{2} \widehat{\vec{d}}_1^B \vec{m}_2^A\right)\transp & \left(-\tfrac{1}{2} \widehat{\vec{d}}_2^B \vec{m}_2^A\right)\transp & \left(-\tfrac{1}{2} \widehat{\vec{d}}_3^B \vec{m}_2^A\right)\transp
              \end{smallmatrix}\right]
    \left[\begin{smallmatrix}
                  \dot{\boldsymbol{\varphi}}^A \\
                  \dot{\vec{d}}_1^A \\
                  \dot{\vec{d}}_2^A \\
                  \dot{\vec{d}}_3^A \\
                  \dot{\boldsymbol{\varphi}}^B \\
                  \dot{\vec{d}}_1^B\\
                  \dot{\vec{d}}_2^B\\
                  \dot{\vec{d}}_3^B
              \end{smallmatrix}\right],
    \label{eq:internal-port-matrix-cylindrical-pair}
\end{align}
where the matrix has the same dimension as $\nabla \vec{g}(\vec{q})$ in \eqref{eq:cylindrical-pair-constraint-jacobian}, so each row can be compared directly.

%########################################################################
\subsection{Translational constraints}
\label{annexsubsec:row1-derivation}
%########################################################################

We begin from row~1 of \eqref{eq:internal-port-matrix-cylindrical-pair}:
\begin{align}
    \dot{\vec{g}}_{\text{J},1}^C (\vec{q})
     & = -\vec{m}_1^{A\top} \dot{\boldsymbol{\varphi}}^A
    -\left[\left(X_i^A \vec{I} - \widehat{\vec{d}}_i^A \Delta \widehat{\vec{p}} \right) \vec{m}_1^A\right]\transp \dot{\vec{d}}_i^A \nonumber \\
     & \quad +\vec{m}_1^{A\top} \dot{\boldsymbol{\varphi}}^B
    + \left(X_i^B  \vec{m}_1^A\right)\transp \dot{\vec{d}}_i^B.
\end{align}
Group terms involving $\vec{m}_1^{A\top}$:
\begin{align}
     & = \vec{m}_1^{A\top} \left( \dot{\boldsymbol{\varphi}}^B + X_i^B \dot{\vec{d}}_i^B
    - \dot{\boldsymbol{\varphi}}^A - X_i^A \dot{\vec{d}}_i^A \right)
    + \left[\left( \widehat{\vec{d}}_i^A \Delta \widehat{\vec{p}} \right) \vec{m}_1^A\right]\transp \dot{\vec{d}}_i^A.
    \label{eq:row1-step1}
\end{align}
Recognizing that $\dot{\boldsymbol{\varphi}}^B + X_i^B \dot{\vec{d}}_i^B - \dot{\boldsymbol{\varphi}}^A - X_i^A \dot{\vec{d}}_i^A = \Delta \dot{\vec{p}}$, we have
\begin{align}
    \dot{\vec{g}}_{\text{J},1}^C (\vec{q})
     & = \vec{m}_1^{A\top} \Delta \dot{\vec{p}}
    + \left(m_1^A\right)_i \left[\left( \widehat{\vec{d}}_i^A \Delta \widehat{\vec{p}} \right) \vec{d}_i^A\right]\transp \dot{\vec{d}}_i^A.
    \label{eq:row1-step2}
\end{align}
We now apply the vector identity
\begin{align}
    \widehat{\vec{a}}\,\widehat{\vec{b}}
     & = \vec{b}\,\vec{a}\transp - (\vec{a}\transp \vec{b})\,\vec{I}
    \label{eq:hat-hat-identity}
\end{align}
to $\widehat{\vec{d}}_i^A \Delta \widehat{\vec{p}}$:
\begin{align}
    \widehat{\vec{d}}_i^A \Delta \widehat{\vec{p}}
     & = \Delta \vec{p} \left(\vec{d}_i^A\right)\transp
    - \left[\left(\vec{d}_i^A\right)\transp \Delta \vec{p}\right]\vec{I}.
    \label{eq:row1-step3}
\end{align}
Substituting \eqref{eq:row1-step3} into the second term of \eqref{eq:row1-step2} yields
\begin{subequations}
    \begin{align}
        \dot{\vec{g}}_{\text{J},1}^C (\vec{q})
         & = \vec{m}_1^{A\top} \Delta \dot{\vec{p}}
        + \left(m_1^A\right)_i
        \left( \Delta \vec{p} \, (\vec{d}_i^A)\transp \vec{d}_i^A
        - \left[(\vec{d}_i^A)\transp \Delta \vec{p}\right] \vec{d}_i^A \right)\transp
        \dot{\vec{d}}_i^A                           \\
         & = \vec{m}_1^{A\top} \Delta \dot{\vec{p}}
        + \left(m_1^A\right)_i
        \left( \Delta \vec{p}\transp \dot{\vec{d}}_i^A
        - \left[(\vec{d}_i^A)\transp \Delta \vec{p}\right] \left[(\vec{d}_i^A)\transp \dot{\vec{d}}_i^A\right] \right).
    \end{align}
\end{subequations}
Since $\vec{d}_i^A$ is a unit vector, $(\vec{d}_i^A)\transp \dot{\vec{d}}_i^A = 0$:
\begin{align}
    \dot{\vec{g}}_{\text{J},1}^C (\vec{q})
     & = \vec{m}_1^{A\top} \Delta \dot{\vec{p}}
    + \left(m_1^A\right)_i \Delta \vec{p}\transp \dot{\vec{d}}_i^A.
\end{align}
Recognizing that $\left(m_1^A\right)_i \dot{\vec{d}}_i^A = \dot{\vec{m}}_1^A$:
\begin{align}
    \dot{\vec{g}}_{\text{J},1}^C (\vec{q})
     & = \vec{m}_1^{A\top} \Delta \dot{\vec{p}}
    + \left( \dot{\vec{m}}_1^A \right)\transp \Delta \vec{p}.
\end{align}

%########################################################################
\subsection{Rotational constraints}
\label{annexsubsec:row3-derivation}
%########################################################################

We start from row~3 of \eqref{eq:internal-port-matrix-cylindrical-pair}:
\begin{align}
    \dot{\vec{g}}_{\text{J},3}^C (\vec{q})
     & = \left(\frac{1}{2} \widehat{\vec{d}}_i^A \vec{m}_1^A \right)\transp \dot{\vec{d}}_i^A
    + \left(-\frac{1}{2} \widehat{\vec{d}}_i^B \vec{m}_1^A \right)\transp \dot{\vec{d}}_i^B.
    \label{eq:row-3-cylindrical}
\end{align}
Applying $\widehat{\vec{a}}\,\vec{b} = \vec{a} \times \vec{b}$:
\begin{align}
     & = \frac{1}{2} \left(\vec{d}_i^A \times \vec{m}_1^A\right)\transp \dot{\vec{d}}_i^A
    - \frac{1}{2} \left(\vec{d}_i^B \times \vec{m}_1^A\right)\transp \dot{\vec{d}}_i^B.
\end{align}
Using $(\vec{a} \times \vec{b})\transp \vec{c} = \vec{a}\transp (\vec{b} \times \vec{c})$:
\begin{align}
     & = \frac{1}{2} \vec{d}_i^{A\top} (\vec{m}_1^A \times \dot{\vec{d}}_i^A)
    - \frac{1}{2} \vec{d}_i^{B\top} (\vec{m}_1^A \times \dot{\vec{d}}_i^B).
\end{align}
Rewriting via $\vec{x}\transp (\vec{y} \times \vec{z}) = \vec{y}\transp (\vec{z} \times \vec{x})$:
\begin{align}
     & = \frac{1}{2} \vec{m}_1^{A\top} (\dot{\vec{d}}_i^A \times \vec{d}_i^A)
    - \frac{1}{2} \vec{m}_1^{A\top} (\dot{\vec{d}}_i^B \times \vec{d}_i^B).
\end{align}
Since $\dot{\vec{d}}_i \times \vec{d}_i = -\vec{d}_i \times \dot{\vec{d}}_i$:
\begin{align}
     & = -\frac{1}{2} \vec{m}_1^{A\top} (\vec{d}_i^A \times \dot{\vec{d}}_i^A)
    + \frac{1}{2} \vec{m}_1^{A\top} (\vec{d}_i^B \times \dot{\vec{d}}_i^B).
\end{align}
Recognizing $\vec{\omega}^A = \frac{1}{2} \dot{\vec{d}}_i^A\times\vec{d}_i^A $:
\begin{align}
     & = \vec{m}_1^{A\top} \vec{\omega}^B - \vec{m}_1^{A\top} \vec{\omega}^A.
\end{align}
Substituting $\vec{m}_1^A = \vec{n}^A \times \vec{d}_1^B$, which is admissible thanks to the cylindrical joint constraints \eqref{eq:cylindrical-pair-constraints}, so that
\begin{subequations}
    \begin{align}
         & = (\vec{n}^A \times \vec{d}_1^B)\transp \vec{\omega}^B
        - (\vec{n}^A \times \vec{d}_1^B)\transp \vec{\omega}^A    \\
         & = \vec{n}^{A\top} (\vec{d}_1^B \times \vec{\omega}^B)
        - (\vec{\omega}^A \times \vec{n}^A)\transp \vec{d}_1^B    \\
         & = -\vec{n}^{A\top} (\vec{\omega}^B \times \vec{d}_1^B)
        - (\vec{\omega}^A \times \vec{n}^A)\transp \vec{d}_1^B.
    \end{align}
\end{subequations}
Recognizing $\vec{\omega}^B \times \vec{d}_1^B = \dot{\vec{d}}_1^B$ and
$\vec{\omega}^A \times \vec{n}^A = \dot{\vec{n}}^A$:
\begin{align}
     & = -\vec{n}^{A\top} \dot{\vec{d}}_1^B - \dot{\vec{n}}^{A\top} \vec{d}_1^B.
\end{align}
Since velocity constraints must vanish, we can flip the sign:
\begin{align}
    \dot{\vec{g}}_{\text{J},3}^C (\vec{q})
     & = \vec{n}^{A\top} \dot{\vec{d}}_1^B + \dot{\vec{n}}^{A\top} \vec{d}_1^B.
    \label{eq:row-3-cylindrical-2}
\end{align}



%########################################################################
%\subsection{Initial values flying cylindrical pair}\label{annexsec:cylindrical_pair_init_values}
%########################################################################
%The independent generalized velocities at $t=0$ for the problem in Section \ref{sec:cylindrical_pair} are given as
%$$
%    \vec{v}_\text{ind} = \begin{bmatrix}
%       \vec{v}_{\varphi}^A &
%      \vec{\omega}^A      &
%     \dot{u}^B           &
%    \dot{\theta}^B
%\end{bmatrix}\transp = \begin{bmatrix}
%    0    &
%    50   &
%    0    &
%    1    &
%    1.5  &
%    0    &
%    35.5 &
%    -100
%\end{bmatrix}\transp.
%$$

%To ensure kinematic consistency with the cylindrical joint constraints, initial velocities are computed from the angular and linear velocity relations
%\begin{align*}
%    \vec{\omega}^B=\vec{\omega}^A + \dot{\theta}^B \vec{n}^A
%\end{align*}
%and
%\begin{align*}
%    \vec{v}_{\varphi}^B = \vec{v}_{\varphi}^A + \vec{\omega}^A \times (\boldsymbol{\varphi}^B - \boldsymbol{\varphi}^A) + \dot{u}^B \vec{n}^A + \dot{\theta}^B \vec{X}^B \times \vec{n}^A.
%\end{align*}

==> includes/annex_tables.tex <==
%########################################################################
\section{Set-up numerical examples}\label{appendix:num_examples}
%########################################################################
%########################################################################
Unless otherwise specified, all components are provided in the inertial frame.
The first three position and velocity components in the vectors correspond to the center of mass of the body, while the remaining nine correspond to the three director vectors.

\subsection{Cylindrical pair}\label{annexsec:slider_crank}

The full simulation set-up is given by:

\begin{table}[H]
    \centering
    \caption{Simulation setup for bodies in cylindrical pair in director formulation}
    \label{tab:cylindrical_pair_setup_bodies}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabularx}{\textwidth}{l X}
        \multicolumn{2}{l}{\textbf{Bodies}}                                                                 \\
        \hline
        \textbf{Index}            & 0                                                                       \\
        \textbf{Mass}             & 4.0                                                                     \\
        \textbf{Inertias}         & [304, 304, 8]                                                           \\
        \textbf{Gravity}          & [0, 0, 0]                                                               \\
        \textbf{Dimensions}       & [4, 4, 30]                                                              \\
        \textbf{Initial position} & [0, 0, 0, 1, 0, 0, 0, 1, 0, 0, 0, 1]                                    \\
        \textbf{Initial velocity} & [0, 50, 0, -0.0, 0.0, 1.5, -0.0, 0.0, -1.0, -1.5, 1.0, 0.0]             \\
        \textbf{Multiplier}       & [0.0, 0.0, 0.0, 0.0, 0.0, 0.0]                                          \\
        \hline
        \textbf{Index}            & 1                                                                       \\
        \textbf{Mass}             & 3.0                                                                     \\
        \textbf{Inertias}         & [18.75, 18.75, 19.5]                                                    \\
        \textbf{Gravity}          & [0, 0, 0]                                                               \\
        \textbf{Dimensions}       & [6, 6, 6]                                                               \\
        \textbf{Initial position} & [0, 0, -11, 1.0, 0.0, 0.0, 0.0, 1.0, 0.0, 0.0, 0.0, 1.0]                \\
        \textbf{Initial velocity} & [16.5, 39.0, 35.5, -0.0, 100.0, 1.5, -100.0, 0.0, -1.0, -1.5, 1.0, 0.0] \\
        \textbf{Multiplier}       & [0.0, 0.0, 0.0, 0.0, 0.0, 0.0]                                          \\
        \hline
    \end{tabularx}
\end{table}

% =========================
% Joints table
% =========================
\begin{table}[H]
    \centering
    \caption{Simulation setup for joint in cylindrical pair in director formulation}
    \label{tab:cylindrical_pair_setup_joints}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabularx}{\textwidth}{l X}
        \multicolumn{2}{l}{\textbf{Joints}}                    \\
        \hline
        \textbf{Type}                            & Cylindrical \\
        \textbf{Constraints}                     & 4           \\
        \textbf{Body indices}                    & [0, 1]      \\
        \textbf{Joint location}                  & [0, 0, 0]   \\
        \textbf{Reference axis (body $A$ local)} & [0, 0, 1]   \\
        \hline
    \end{tabularx}
\end{table}


%########################################################################
\subsection{Closed loop multibody system}\label{annexsec:closed_loop_MBS}
%########################################################################
The setup for the closed loop multibody system in Section \ref{sec:closed_loop_MBS} is given by:
\begin{table}[H]
    \centering
    \caption{Simulation setup for bodies in closed loop multibody system (in director formulation)}
    \label{tab:bodies_rigid_body_directors_multibody_ph}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabularx}{\textwidth}{l X}
        \multicolumn{2}{l}{\textbf{Bodies}}                               \\
        \hline
        \textbf{Index}            & 0                                     \\
        \textbf{Mass}             & 10.0                                  \\
        \textbf{Inertias}         & [84.1667, 1.6667, 84.1667]            \\
        \textbf{Gravity}          & [0, 0, 0]                             \\
        \textbf{Dimensions}       & [1, 10, 1]                            \\
        \textbf{Initial position} & [5, 0, 0, 1, 0, 0, 0, 1, 0, 0, 0, 1]  \\
        \textbf{Initial velocity} & [0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0]  \\
        \textbf{Multiplier}       & [0, 0, 0, 0, 0, 0]                    \\
        \hline
        \textbf{Index}            & 1                                     \\
        \textbf{Mass}             & 10.0                                  \\
        \textbf{Inertias}         & [1.6667, 84.1667, 84.1667]            \\
        \textbf{Gravity}          & [0, 0, 0]                             \\
        \textbf{Dimensions}       & [10, 1, 1]                            \\
        \textbf{Initial position} & [0, 5, 0, 1, 0, 0, 0, 1, 0, 0, 0, 1]  \\
        \textbf{Initial velocity} & [0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0]  \\
        \textbf{Multiplier}       & [0, 0, 0, 0, 0, 0]                    \\
        \hline
        \textbf{Index}            & 2                                     \\
        \textbf{Mass}             & 10.0                                  \\
        \textbf{Inertias}         & [84.1667, 1.6667, 84.1667]            \\
        \textbf{Gravity}          & [0, 0, 0]                             \\
        \textbf{Dimensions}       & [1, 10, 1]                            \\
        \textbf{Initial position} & [-5, 0, 0, 1, 0, 0, 0, 1, 0, 0, 0, 1] \\
        \textbf{Initial velocity} & [0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0]  \\
        \textbf{Multiplier}       & [0, 0, 0, 0, 0, 0]                    \\
        \hline
        \textbf{Index}            & 3                                     \\
        \textbf{Mass}             & 10.0                                  \\
        \textbf{Inertias}         & [1.6667, 84.1667, 84.1667]            \\
        \textbf{Gravity}          & [0, 0, 0]                             \\
        \textbf{Dimensions}       & [10, 1, 1]                            \\
        \textbf{Initial position} & [0, -5, 0, 1, 0, 0, 0, 1, 0, 0, 0, 1] \\
        \textbf{Initial velocity} & [0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0]  \\
        \textbf{Multiplier}       & [0, 0, 0, 0, 0, 0]                    \\
        \hline
    \end{tabularx}
\end{table}

% =========================
% Joints table
% =========================
\begin{table}[H]
    \centering
    \caption{Simulation setup for joints in closed loop multibody system (in director formulation)}
    \label{tab:joints_rigid_body_directors_multibody_ph}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabularx}{\textwidth}{l X}
        \multicolumn{2}{l}{\textbf{Joints}}   \\
        \hline
        \textbf{Type}           & Spherical   \\
        \textbf{Body indices}   & [0, 1]      \\
        \textbf{Joint location} & [5, 5, 0]   \\
        \hline
        \textbf{Type}           & Spherical   \\
        \textbf{Body indices}   & [1, 2]      \\
        \textbf{Joint location} & [-5, 5, 0]  \\
        \hline
        \textbf{Type}           & Spherical   \\
        \textbf{Body indices}   & [2, 3]      \\
        \textbf{Joint location} & [-5, -5, 0] \\
        \hline
        \textbf{Type}           & Spherical   \\
        \textbf{Body indices}   & [3, 0]      \\
        \textbf{Joint location} & [5, -5, 0]  \\
        \hline
    \end{tabularx}
\end{table}

%########################################################################
\subsection{Spatial slider-crank mechanism}\label{annexsec:slider_crank}
%########################################################################

Initial velocities in Section \ref{sec:slider_crank_mechanism} are calculated by solving the linear system of equations
\begin{subequations}
    \begin{align}
        \vec{v}^{BC} - \vec{\omega}^{BC} \times \vec{\rho}^{BC} - \vec{v}^{\text{block}}                                & = 0 \\
        \vec{v}^{BC} - \vec{v}^{AB} + \vec{\omega}^{AB} \times \vec{\rho}^{AB} - \vec{\omega}^{BC} \times \vec{\rho}^{BC} & = 0 \\
        \left(\vec{\omega}^{BC}\times\vec{d}_3^{BC}\right)\transp \vec{n}^{\text{block}}                                 & = 0
    \end{align}
\end{subequations}
based on the kinematic joint constraints. It should be noted that due to the nature of the joint configuration, it is not trivial to determine initial conditions, as the rotational constraints must always be
orthogonal to the normal vector defined in the set-up.

The full simulation set-up is given by:

\begin{table}[H]
    \centering
    \caption{Simulation setup for bodies in spatial slider-crank mechanism (director formulation)}
    \label{tab:slider_crank_setup_bodies}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabularx}{\textwidth}{l X}
        \multicolumn{2}{l}{\textbf{Bodies}}                                                                                               \\
        \hline
        \textbf{Index}            & 0                                                                                                     \\
        \textbf{Mass}             & 0.12                                                                                                  \\
        \textbf{Inertias}         & [0.0001, 0.0001, 0.00001]                                                                             \\
        \textbf{Gravity}          & [0, 0, -9.81]                                                                                         \\
        \textbf{Dimensions}       & [0.01, 0.01, 0.08]                                                                                    \\
        \textbf{Initial position} & [0, 0.1, 0.16, 1, 0, 0, 0, 1, 0, 0, 0, 1]                                                             \\
        \textbf{Initial velocity} & [0.0, -0.24, -0.0, 0.0, 0.0, 0.0, 0.0, 0.0, 6.0, 0.0, -6.0, 0.0]                                      \\
        \textbf{Multiplier}       & [0.0, 0.0, 0.0, 0.0, 0.0, 0.0]                                                                        \\
        \hline
        \textbf{Index}            & 1                                                                                                     \\
        \textbf{Mass}             & 0.5                                                                                                   \\
        \textbf{Inertias}         & [0.004, 0.0004, 0.004]                                                                                \\
        \textbf{Gravity}          & [0, 0, -9.81]                                                                                         \\
        \textbf{Dimensions}       & [0.01, 0.3, 0.01]                                                                                     \\
        \textbf{Initial position} & [0.1, 0.05, 0.1, 0.745356, 0.298142, 0.596285, -0.666667, 0.333333, 0.666667, 0, -0.894427, 0.447214] \\
        \textbf{Initial velocity} & [0.12, -0.24, 0.0, -0.715542, -0.787096, 1.287975, -0.8, -1.6, 0, 0, -0.85865, -1.7173]               \\
        \textbf{Multiplier}       & [0.0, 0.0, 0.0, 0.0, 0.0, 0.0]                                                                        \\
        \hline
        \textbf{Index}            & 2                                                                                                     \\
        \textbf{Mass}             & 2.0                                                                                                   \\
        \textbf{Inertias}         & [0.0001, 0.0001, 0.0001]                                                                              \\
        \textbf{Gravity}          & [0, 0, -9.81]                                                                                         \\
        \textbf{Dimensions}       & [0.03, 0.03, 0.03]                                                                                    \\
        \textbf{Initial position} & [0.2, 0, 0, 1, 0, 0, 0, 1, 0, 0, 0, 1]                                                                \\
        \textbf{Initial velocity} & [0.24, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0]                                                               \\
        \textbf{Multiplier}       & [0.0, 0.0, 0.0, 0.0, 0.0, 0.0]                                                                        \\
        \hline
    \end{tabularx}
\end{table}

% =========================
% Joints table
% =========================
\begin{table}[H]
    \centering
    \caption{Simulation setup for joints in spatial slider-crank mechanism (director formulation)}
    \label{tab:slider_crank_setup_joints}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabularx}{\textwidth}{l X}
        \multicolumn{2}{l}{\textbf{Joints}}                     \\
        \hline
        \textbf{Type}                          & Revolute       \\
        \textbf{Constraints}                   & 5              \\
        \textbf{Body indices}                  & [0, 0]         \\
        \textbf{Joint location}                & [0, 0.1, 0.12] \\
        \textbf{Reference axis (body A local)} & [1, 0, 0]      \\
        \hline
        \textbf{Type}                          & Spherical      \\
        \textbf{Constraints}                   & 3              \\
        \textbf{Body indices}                  & [0, 1]         \\
        \textbf{Joint location}                & [0, 0.1, 0.2]  \\
        \hline
        \textbf{Type}                          & Universal      \\
        \textbf{Constraints}                   & 4              \\
        \textbf{Body indices}                  & [2, 1]         \\
        \textbf{Joint location}                & [0.2, 0, 0]    \\
        \textbf{Reference axis (body A local)} & [1, 0, 0]      \\
        \hline
        \textbf{Type}                          & Prismatic      \\
        \textbf{Constraints}                   & 5              \\
        \textbf{Body indices}                  & [2, 2]         \\
        \textbf{Joint location}                & [0.2, 0, 0]    \\
        \textbf{Reference axis (body A local)} & [1, 0, 0]      \\
        \hline
    \end{tabularx}
\end{table}




